Brownian Molecules Formed by Delayed Harmonic Interactions

A time-delayed response of individual living organisms to information exchanged within flocks or swarms leads to the emergence of complex collective behaviors. A recent experimental setup by (Khadka et al 2018 Nat. Commun. 9 3864), employing synthetic microswimmers, allows to emulate and study such behavior in a controlled way, in the lab. Motivated by these experiments, we study a system of N Brownian particles interacting via a retarded harmonic interaction. For $N \leq 3$ , we characterize its collective behavior analytically, by solving the pertinent stochastic delay-differential equations, and for $N>3$ by Brownian dynamics simulations. The particles form molecule-like non-equilibrium structures which become unstable with increasing number of particles, delay time, and interaction strength. We evaluate the entropy and information fluxes maintaining these structures and, to quantitatively characterize their stability, develop an approximate time-dependent transition-state theory to characterize transitions between different isomers of the molecules. For completeness, we include a comprehensive discussion of the analytical solution procedure for systems of linear stochastic delay differential equations in finite dimension, and new results for covariance and time-correlation matrices.

==> Content/Titlepage.tex <==
\begin{abstract}
A time-delayed response of individual living organisms to information exchange within groups or swarms leads to the formation of complex collective behaviors. A recent experimental setup by Khadka et al., Nat. Commun. {\bf 9}, 3864 (2018), employing synthetic microswimmers, allows to realize and study such behavior in a controlled way, in the lab. Motivated by these experiments, we study a system of $N$ Brownian particles interacting via a harmonic, time-delayed potential. For $N \le 3$, we model the problem analytically by systems of linear stochastic delay differential equations, and for $N > 3$ we use Brownian dynamics simulations. The particles form molecular-like structures which become increasingly unstable with the number of particles and the length of the delay. We evaluate the entropy fluxes in the system and develop an appropriate time-dependent transition state theory to characterize transitions between different isomers of the molecules. In the appendix, we provide an extensive review of the analytical solution of systems of linear stochastic delay differential equations in an arbitrary dimension and include new results for covariance and time-correlation matrices.
%	Many living organisms perform some sort of collective behavior controlled by an appropriate exchange of information. Recently, Khadka et al. \cite{khadka2018active} presented an experimental setup for a system of Brownian particles which interact -- based on optical feedback techniques -- via time delayed forces. As such a time delay may also arise in biological systems due to a finite time of information processing, we investigate on its effects on collective dynamics. Therefore, we adapt the basic model of \cite{khadka2018active} and study a system of $N$ Brownian particles interacting via a harmonic, time-delayed potential. Under certain approximations this problem can be modeled by linear stochastic delay differential equations from which the time-dependent solution for the 1- and 2-time probability distribution is derived. The systems form molecular-like structures which, depending on the number of particles and the size of the delay, become increasingly unstable. The entropy of the total system is evaluated and an appropriate time dependent transition state theory is formulated to characterize the transitions between different configurations. It is should be emphasized that our analysis also applies to system of kinds of delay or memory kernels.
\end{abstract}

%\textbf{Keywords:} Stochastic Delay Differential Equation, Active Matter, Feedback Driving, Non-Markovian Dynamics, Fokker-Planck Eq., Structure Formation, Transition-State Theory 

\maketitle


\tableofcontents


	


